About presentations of braid groups and their generalizations

In the paper we give a survey of rather new notions and results which generalize classical ones in the theory of braids. Among such notions are various inverse monoids of partial braids. We also observe presentations different from standard Artin presentation for generalizations of braids. Namely, we consider presentations with small number of generators, Sergiescu graph-presentations and Birman-Ko-Lee presentation. The work of V.V.Chaynikov on the word and conjugacy problems for the singular braid monoid in Birman-Ko-Lee generators is described as well.

==> weld.tex <==
\begin{picture}(0,50)(0,-5) 
%\centerline{\noindent\latexpic(0,50)(0,-5) \thicklines
\put(0,20){\circle*{5}} \put(-10,40){\line(1,-2){20}}
\put(10,40){\line(-1,-2){20}}
%\endlatexpic}
\end{picture}
%\centerline{Fig. 5.2} \vglue 0.5cm
